KAER: A Knowledge Augmented Pre-Trained Language Model for Entity Resolution

Entity resolution has been an essential and well-studied task in data cleaning research for decades. Existing work has discussed the feasibility of utilizing pre-trained language models to perform entity resolution and achieved promising results. However, few works have discussed injecting domain knowledge to improve the performance of pre-trained language models on entity resolution tasks. In this study, we propose Knowledge Augmented Entity Resolution (KAER), a novel framework named for augmenting pre-trained language models with external knowledge for entity resolution. We discuss the results of utilizing different knowledge augmentation and prompting methods to improve entity resolution performance. Our model improves on Ditto, the existing state-of-the-art entity resolution method. In particular, 1) KAER performs more robustly and achieves better results on "dirty data", and 2) with more general knowledge injection, KAER outperforms the existing baseline models on the textual dataset and dataset from the online product domain. 3) KAER achieves competitive results on highly domain-specific datasets, such as citation datasets, requiring the injection of expert knowledge in future work.

==> 04table1.tex <==

\begin{table*}[!ht]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ll|llll|l}
\hline
\multicolumn{1}{l|}{}                  & \multicolumn{2}{c|}{\textbf{Dirty}} & \multicolumn{4}{c|}{\textbf{Structured}}                      & \textbf{Textual} \\ \hline
\multicolumn{1}{l|}{\textbf{Models}} &
  \textbf{\begin{tabular}[l]{@{}l@{}}DBLP\\ -\\ GoogleScholar\end{tabular}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[l]{@{}l@{}}iTunes\\ -\\ Amazon\end{tabular}}} &
  \textbf{\begin{tabular}[l]{@{}l@{}}iTunes\\ -\\ Amazon\end{tabular}} &
  \textbf{\begin{tabular}[l]{@{}l@{}}Amazon\\ -\\ Google\end{tabular}} &
  \textbf{\begin{tabular}[l]{@{}l@{}}DBLP\\ -\\ ACM\end{tabular}} &
  \multicolumn{1}{l|}{\textbf{\begin{tabular}[l]{@{}l@{}}DBLP\\ -\\ GoogleScholar\end{tabular}}} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Abt\\ -\\ Buy\end{tabular}} \\ \hline
RoBERTa                          & 98.42                             & 86.24                       & 76.15                       & 94.55                       & 99.56                   & 98.26                             & 97.49                                \\
Ditto                            & 98.35                             & 80.73                       & 75.23                       & 94.07                       & 99.47                   & 98.45                             & 97.65                                \\ \hline
KAER ( Roberta + CST )           & 98.31                             & 81.65                       & 89.91**++                   & 93.72                       & 99.56                   & 98.19                             & 98.38**++                            \\
KAER ( Roberta + CST + / )       & 98.40                              & 78.90*                       & \textbf{94.50**++}           & 94.64                       & \textbf{99.64}          & 98.21                             & \textbf{98.43**++}                   \\
KAER ( Roberta + CST + PCT)      & 98.22                             & 87.16                       & 72.48                       & \textbf{94.81}              & 99.31*                  & 98.35                             & 95.62**++                            \\
KAER ( Roberta + EL )            & 98.15                             & 77.98*                      & 81.65                       & 94.64                       & 99.47                   & 98.40                              & 97.70                                 \\
KAER ( Roberta + EL + / )        & 98.43                   & \textbf{88.99}              & 92.66**++                   & 94.24                       & 99.43                   & \textbf{98.55*}                   & 97.44                                \\
KAER ( Roberta + EL + PCT)       & 98.03**+                          & \textbf{88.99+}             & 80.73                       & 94.55                       & 98.95**+                & 98.24                             & 94.89**++                            \\
KAER ( Roberta + CST + EL )      & \textbf{98.45}                    & 75.23*                      & 79.82                       & 94.11                       & 99.43                   & 98.36                             & 97.81                                \\
KAER ( Roberta + CST + EL + / )  & 98.36                             & 79.82*                      & 80.73+                      & 94.55                       & 99.39                   & 98.36                             & 97.70                                 \\
KAER ( Roberta + CST + EL + PCT) & 97.82**++                         & 88.07+                      & 77.98                       & 93.63*                      & 98.67**++               & 98.10+                             & 93.58**++                            \\ \hline
\end{tabular}
}
\vspace{-0.4cm}
\caption{Experimental results using different knowledge injection methods, measured by accuracy. 
% 99\% and 95\% confidence level of hypothesis test (paired t-test).
The two baseline models: RoBERTa (without domain knowledge injection); and Ditto (RoBERTa and Ditto's general domain knowledge injection methods). 
% representing the baseline model, Ditto without knowledge injection, 
Other models represent KAER with various knowledge injection and prompting methods combined with RoBERTa. ``+CST'' indicates \textbf{C}olumn \textbf{S}emantic \textbf{T}ype injection.``+EL'' indicates knowledge injection with \textbf{E}ntity \textbf{L}inking. ``+/'' represents prompting with a slash. ``+PCT'' represents \textbf{P}rompting with \textbf{C}onstrained \textbf{T}uning, i.e., soft positions and visible matrix. The paired t-test is processed between KAER injections and two baseline models, i.e., RoBERTa(*) and Ditto(+). \textbf{**} and \textbf{++} represent 99\% confidence level, and \textbf{*} and \textbf{+} represent 95\% confidence level.}%significance level ($\alpha=0.05$).} 
\label{tab:injection_results}
\vspace{-0.5cm}
\end{table*}

% \begin{table*}[!ht]
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|ll|llll|l}
% \hline
% \multicolumn{1}{l|}{}                  & \multicolumn{2}{c|}{\textbf{Dirty}} & \multicolumn{4}{c|}{\textbf{Structured}}                      & \textbf{Textual} \\ \hline
% \multicolumn{1}{l|}{\textbf{Models}} &
%   \textbf{\begin{tabular}[l]{@{}l@{}}DBLP\\ -\\ GoogleScholar\end{tabular}} &
%   \multicolumn{1}{c|}{\textbf{\begin{tabular}[l]{@{}l@{}}iTunes\\ -\\ Amazon\end{tabular}}} &
%   \textbf{\begin{tabular}[l]{@{}l@{}}iTunes\\ -\\ Amazon\end{tabular}} &
%   \textbf{\begin{tabular}[l]{@{}l@{}}Amazon\\ -\\ Google\end{tabular}} &
%   \textbf{\begin{tabular}[l]{@{}l@{}}DBLP\\ -\\ ACM\end{tabular}} &
%   \multicolumn{1}{l|}{\textbf{\begin{tabular}[l]{@{}l@{}}DBLP\\ -\\ GoogleScholar\end{tabular}}} &
%   \textbf{\begin{tabular}[c]{@{}l@{}}Abt\\ -\\ Buy\end{tabular}} \\ \hline
% RoBERTa                          & 95.81                             & 72.73                       & 61.76                       & 73.12                       & 98.77                   & 95.32                             & 88.41                                \\
% Ditto                            & 95.54**                           & 60.38                       & 47.06**                     & 74.44**                     & 98.55*                  & 95.85                             & 88.89                                \\ \hline
% KAER ( RoBERTa + CST )           & 95.47**                           & 62.96                       & 80.70*                      & 68.70++                   & 98.77+                 & 95.05**++                       & 92.27*                               \\
% KAER ( RoBERTa + CST + / )       & 95.74++                         & 54.90                       & \textbf{89.66}              & 74.85*++                  & \textbf{98.99+}        & 95.14*++                        & \textbf{92.61}                       \\
% KAER ( RoBERTa + CST + PCT)      & 95.20**                           & 72.00                       & 57.14++                   & \textbf{76.25**++}        & 98.09+                 & 95.62**++                       & 78.24**+                            \\
% KAER ( RoBERTa + EL )            & 95.12++                         & 50.00                       & 61.54**                     & 73.77++                   & 98.54++               & 95.72                             & 89.11*                               \\
% KAER ( RoBERTa + EL + / )        & 95.75**                           & \textbf{81.82**++}        & 86.21                       & 74.02**+                   & 98.43++               & \textbf{96.11}                    & 88.19                                \\
% KAER ( RoBERTa + EL + PCT)       & 94.80++                         & 77.78                       & 67.69+                     & 75.63**+                   & 97.04**++             & 95.29                             & 73.80**++                          \\
% KAER ( RoBERTa + CST + EL )      & \textbf{95.87*++}               & 47.06                       & 59.26**                     & 72.28*++                  & 98.43+                 & 95.65**++                       & 89.66                                \\
% KAER ( RoBERTa + CST + EL + / )  & 95.63*++                        & 63.33+                     & 57.14**                     & 75.15**++                 & 98.34*                  & 95.67**++                       & 89.81**++                          \\
% KAER ( RoBERTa + CST + EL + PCT) & 94.24++                         & 71.11**+                   & 61.29+                     & 71.37**+                   & 96.26+                 & 94.93                             & 67.20**++                          \\ \hline
% \end{tabular}
% }
% \vspace{-0.2cm}
% \caption{Experimental results using different knowledge injection methods. 
% % 99\% and 95\% confidence level of hypothesis test (paired t-test).
% The two baseline models: RoBERTa (without domain knowledge injection); and Ditto (RoBERTa and Ditto's general domain knowledge injection methods). 
% % representing the baseline model, Ditto without knowledge injection, 
% Other models represent KAER with various knowledge injection and prompting methods combined with RoBERTa. ``+CST'' indicates \textbf{C}olumn \textbf{S}emantic \textbf{T}ype injection.``+EL'' indicates knowledge injection with \textbf{E}ntity \textbf{L}inking. ``+/'' represents prompting with a slash. ``+PCT'' represents \textbf{P}rompting with \textbf{C}onstrained \textbf{T}uning, i.e., soft positions and visible matrix. All reported results are F1 scores. The paired t-test is processed between KAER injections and two baseline models, i.e., RoBERTa(*) and Ditto(+). \textbf{**} and \textbf{++} represent 99\% confidence level, and \textbf{*} and \textbf{+} represent 95\% confidence level.}%significance level ($\alpha=0.05$).} 
% \label{tab:injection_results}
% \end{table*}

% \begin{table*}[!ht]
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|cc|cccc|c}
% \hline
% \multicolumn{1}{l|}{}                  & \multicolumn{2}{c|}{\textbf{Dirty}} & \multicolumn{4}{c|}{\textbf{Structured}}                      & \textbf{Textual} \\ \hline
% \multicolumn{1}{c|}{\textbf{Injection}} &
%   \textbf{\begin{tabular}[c]{@{}c@{}}DBLP\\ -\\ GoogleScholar\end{tabular}} &
%   \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}iTunes\\ -\\ Amazon\end{tabular}}} &
%   \textbf{\begin{tabular}[c]{@{}c@{}}iTunes\\ -\\ Amazon\end{tabular}} &
%   \textbf{\begin{tabular}[c]{@{}c@{}}Amazon\\ -\\ Google\end{tabular}} &
%   \textbf{\begin{tabular}[c]{@{}c@{}}DBLP\\ -\\ ACM\end{tabular}} &
%   \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}DBLP\\ -\\ GoogleScholar\end{tabular}}} &
%   \textbf{\begin{tabular}[c]{@{}c@{}}Abt\\ -\\ Buy\end{tabular}} \\ \hline
% RoBERTa                            & 95.8            & 66.7              & 85.2          & 73.2          & \textbf{98.8} & 95.9          & 88.4             \\
% Ditto    & 95.2            & 77.1              & 53.8          & 76.7          & 98.6          & 95.9          & 88.9             \\ \hline
% KAER (RoBERTa + CST)             & 95.8            & \textbf{90.2}     & \textbf{92.6} & 67.3          & \textbf{98.8} & 94.3          & 89.2             \\
% KAER (RoBERTa + CST + /)          & 95.7            & 90.0                & 88.9          & 70.0            & 98.7          & 95.5          & \textbf{91.7}    \\
% KAER (RoBERTa + CST + APE)     & 95.3            & 66.7              & 66.7          & \textbf{77.9} & 97.5          & 95.7          & 77.2             \\
% KAER (RoBERTa + EL)                      & 95.6            & 87.3              & 72.4          & 73.5          & 98.5          & 95.5          & 89.1             \\
% KAER (RoBERTa + EL + /)                   & 95.5            & 80.8              & 84.6          & 73.1          & 98.4          & \textbf{96.2} & 88.2             \\
% KAER (RoBERTa + EL + APE)             & 95.2            & 80.9              & 69.7          & 76.2          & 97.1          & 95.3          & 74.8             \\
% KAER (RoBERTa + CST + EL)       & 95.7            & 69.7              & 73.5          & 71.7          & 98.4          & \textbf{96.2} & 89.7             \\
% KAER (RoBERTa + CST + EL + /)    & \textbf{96.0}     & 75.4              & 61.5          & 75.5          & 98.3          & 95.2          & 89.8             \\
% KAER (RoBERTa + CST + EL + APE) & 94.8            & 66.7              & 70.0          & 73.5          & 96.5          & 94.7          & 66.8             \\ \hline
% \end{tabular}
% }
% \vspace{-0.2cm}
% \caption{Experimental results using different knowledge injection methods. All reported results are F1 scores. The two baseline models include RoBERTa without domain knowledge injection (in row 1) and Ditto with RoBERTa and its general domain knowledge injection methods (in row 2). 
% % representing the baseline model, Ditto without knowledge injection, 
% Subsequent rows represent the various knowledge injection and prompting methods combined with RoBERTa. ``+CST'' indicates \textbf{C}olumn \textbf{S}emantic \textbf{T}ype injection.``+EL'' indicates knowledge injection with \textbf{E}ntity \textbf{L}inking. ``+/'' represents prompting with a slash. ``+APE'' represents prompting with \textbf{A}dditional \textbf{P}osition \textbf{E}ncoding, i.e., soft positions and visible matrix.}
% \label{tab:injection_results}
% \vspace{-0.5cm}
% \end{table*}

% % \begin{table*}[!ht]
% % \centering
% % \resizebox{\linewidth}{!}{
% % \begin{tabular}{lccccccc}
% % \hline
% % \multicolumn{1}{l|}{}                  & \multicolumn{2}{c|}{\textbf{Dirty}} & \multicolumn{4}{c|}{\textbf{Structured}}                      & \textbf{Textual} \\ \hline
% % \multicolumn{1}{c|}{\textbf{Injection}} &
% %   \textbf{\begin{tabular}[c]{@{}c@{}}DBLP\\ -\\ GoogleScholar\end{tabular}} &
% %   \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}iTunes\\ -\\ Amazon\end{tabular}}} &
% %   \textbf{\begin{tabular}[c]{@{}c@{}}iTunes\\ -\\ Amazon\end{tabular}} &
% %   \textbf{\begin{tabular}[c]{@{}c@{}}Amazon\\ -\\ Google\end{tabular}} &
% %   \textbf{\begin{tabular}[c]{@{}c@{}}DBLP\\ -\\ ACM\end{tabular}} &
% %   \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}DBLP\\ -\\ GoogleScholar\end{tabular}}} &
% %   \textbf{\begin{tabular}[c]{@{}c@{}}Abt\\ -\\ Buy\end{tabular}} \\ \hline
% % \textbf{Ditto} (baseline)                         & 95.8             & 66.7             & 85.2          & 73.2          & \textbf{98.8}          & 95.9          & 88.4             \\
% % \textbf{Ditto + Sherlock}              & 95.8             & \textbf{90.2}    & \textbf{92.6} & 67.3          & \textbf{98.8}          & 94.3          & 89.2             \\
% % \textbf{Ditto + Sherlock + /}          & 95.7             & 90.0             & 88.9          & 70.0          & 98.7          & 95.5          & \textbf{91.7}             \\
% % \textbf{Ditto + Sherlock + KBert}      & 95.3             & 66.7             & 66.7          & \textbf{77.9}          & 97.5          & 95.7          & 77.2             \\
% % % \textbf{Ditto + Doduo}                 & 94.8             & 88.5             & 66.7          & 72.5          & 98.8          & 95.6          & 88.6             \\
% % % \textbf{Ditto + Doduo + /}             & 95.4             & 80.0             & 53.6          & 76.6 & 98.8          & 95.7          & 88.9             \\
% % % \textbf{Ditto + Doduo + KBert}         & 95.5             & 72.0             & 72.7          & 75.4          & 96.9          & 95.6          & 69.4             \\
% % \textbf{Ditto + EL}                    & 95.6             & 87.3             & 72.4          & 73.5          & 98.5          & 95.5          & 89.1             \\
% % \textbf{Ditto + EL + /}                & 95.5             & 80.8             & 84.6          & 73.1          & 98.4          & \textbf{96.2} & 88.2             \\
% % \textbf{Ditto + EL + KBert}            & 95.2             & 80.9             & 69.7          & 76.2          & 97.1          & 95.3          & 74.8             \\
% % \textbf{Ditto + Sherlock + EL}         & 95.7             & 69.7             & 73.5          & 71.7          & 98.4          & \textbf{96.2} & 89.7             \\
% % \textbf{Ditto + Sherlock + EL + /}     & \textbf{96.0}    & 75.4             & 61.5          & 75.5          & 98.3          & 95.2          & 89.8             \\
% % \textbf{Ditto + Sherlock + EL + KBert} & 94.8             & 66.7             & 70.0          & 73.5          & 96.5          & 94.7          & 66.8             \\
% % % \textbf{Ditto + Doduo + EL}            & 95.2             & 62.5             & 66.7          & 74.4          & \textbf{99.0} & 95.8          & \textbf{92.1}    \\
% % % \textbf{Ditto + Doduo + EL + /}        & 95.3             & 62.5             & 54.5          & 75.5          & 98.8          & 95.4          & 89.0             \\
% % % \textbf{Ditto + Doduo + EL + KBert}    & 94.1             & 69.2             & 71.7          & 76.2          & 95.8          & 94.9          & 56.7             \\ 
% % \hline
% % \end{tabular}
% % }
% % \caption{Results using different knowledge injection methods. All reported results are F1 scores. The first line represents the baseline model, Ditto without knowledge injection, and the subsequent rows represent the various knowledge injection and prompting methods combined with Ditto. "+Sherlock" indicates column semantic type prediction. "+EL" indicates knowledge injection with entity linking. "+/" represents prompting with a slash. "+KBert" represents prompting with additional position encoding, i.e., soft positions and visible matrix.}
% % \label{tab:injection_results}
% % \end{table*}

==> 10experiment-copy.tex <==
% TODO: dataset statistic table
\subsection{Dataset}

KAER is evaluated on the Magellan datasets \cite{magellandata} across various domains. 
%The data collection contains datasets designed for entity matching tasks . 
The overview of the datasets used in this study is shown in Table~\ref{tab:dataset_overview}. 
The Magellan datasets contain three types of datasets: dirty dataset, structured dataset, and textual dataset.
The dirty dataset is generated from the structured dataset by randomly removing attribute values and appending the initial values to another randomly selected attribute~\cite{li_deep_2020}.

\begin{table}[h]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lclccc}
\hline
\textbf{Data Type} & \textbf{Dataset} & \textbf{Domain} & \textbf{Size} & \textbf{\# Positive} & \textbf{\# Attr.} \\ \hline
Structured             & Amazon-Google      & software & 11,460 & 1,167 & 3 \\
                       & iTunes-Amazon      & music    & 539    & 132   & 8 \\
                       & DBLP-ACM           & citation & 12,363 & 2,220 & 4 \\
                       & DBLP-GoogleScholar & citation & 28,707 & 5,347 & 4 \\ \hline
\multirow{3}{*}{Dirty} & iTunes-Amazon      & music    & 539    & 132   & 8 \\
                       & DBLP-ACM           & citation & 12,363 & 2,220 & 4 \\
                       & DBLP-GoogleScholar & citation & 28,707 & 5,347 & 4 \\ \hline
Textual                & Abt-Buy            & product  & 9,575  & 1,028 & 3 \\ \hline
\end{tabular}
}
\caption{Dataset Summary}
\label{tab:dataset_overview}
\vspace{-0.5cm}
\end{table}

% \subsection{Implementation Details}
% We use RoBERTa-base as the backbone model. 
\subsection{Results}
The experimental results are presented in Table \ref{tab:injection_results}.

\textit{Knowledge augmentation performs better on smaller datasets.}
According to the experimental results, incorporating external knowledge can improve the performance on entity resolution tasks. In particular, the proposed knowledge augmentation methods outperform the two baseline models in a data-scarce context.
% This improvement is found to be more significant on datasets with a smaller amount of training data. 
% The results show that our proposed knowledge augmentation methods can improve the model performance over the state-of-the-art Ditto model, especially in a data-scarce context. 
% the F1 score of most knowledge injection methods and prompting methods are higher than the F1 score of baseline model Ditto 
For example, \textbf{KAER (RoBERTa+EL+/)} outperforms both baseline models Roberta and Ditto by 9.09\% and 21.44\% $\uparrow$ on dataset Dirty/iTunes-Amazon significantly and 24.45\% and 39.15\% $\uparrow$ on dataset Structured/iTunes-Amazon. The two baseline models perform worse on smaller datasets because the language model might not be able to learn enough information to distinguish between different entities when fine tuning, given fewer training instances correctly. 
 % \textit{Prompting with "/" performs better than space and K-BERT style injection.}
% Through prompting, the model is provided with additional knowledge to augment the learning process. The experimental results revealed that using slash ``/'' to prompt the model with additional knowledge performs better than using space and \textbf{P}rompting with \textbf{C}onstrained \textbf{T}uning (PCT) in most scenarios. For example, \textbf{KAER (RoBERTa+EL+/)} performs better than the other two prompting methods 
% %space and APE \textbf{KAER (RoBERTa+CST+EL)} and \textbf{KAER(RoBERTa+CST+EL+APE)} 
% on dataset Structured/DBLP-GoogleScholar. 
Prompting with PCT achieves better performance in datasets with smaller text lengths. For example, \textbf{KAER (RoBERTa+CST+PCT)} reaches the best F1 score (76.25\%) on dataset Structured/Amazon-Google, which contains the smallest length of serialized data entry. Moreover, with the test statistic higher than the t value with $\alpha=0.01$, \textbf{KAER (RoBERTa+CST+PCT)} on Structured/Amazon-Google makes a significant difference compared to both baseline models, at 99\% confidence level.

\textit{Knowledge augmentation does not perform well on datasets from certain domains.}
The datasets used in our experiments span several different domains. Using our proposed knowledge augmentation methods (CST and EL), records from certain domains, such as music and online product, benefit from more accurate retrieved knowledge.
For example, \textbf{KAER (RoBERTa+CST+/)} achieves the best F1-score, i.e., 92.61\%, on the textual dataset Abt-Buy from the online product domain.
\textbf{KAER (RoBERTa+EL+/)} achieves the best F1-score (81.82\%) on the musical dataset Dirty/iTunes-Amazon. %As analyzed above, it outperforms both baseline models significantly. 
One potential reason for this notable improvement is that the entities mentioned in the datasets from these domains are more general.
However, publication datasets from domains like citation require more domain-specific or even expert knowledge rather than general commonsense. Our knowledge injection methods are primarily designed for retrieving general knowledge.
Thus, for datasets, like Structured/DBLP-ACM, \textbf{KAER (RoBERTa+CST)} performs as well as Roberta and significantly makes a difference with Ditto at 95\% confidence level, and \textbf{KAER (RoBERTa+CST)+/}  achieves the best F1-score 98.99\%. But all the other KAER models perform worse. For future improvement, additional external expert knowledge from the citation domain should be incorporated for knowledge injection. 
% \vt{The knowledge injection does not help in the highly domain-specific dataset. The knowledge we inject is not the correct knowledge in terms of the domain.}

\textit{Knowledge augmentation is affected by data quality.}
%We notice that 
KAER, with certain knowledge augmentation methods, outperforms the baseline models on dirty datasets. For instance, \textbf{KAER (RoBERTa+CST+EL)} slightly exceeds RoBERTa, and Ditto on Dirty/DBLP-GoogleScholar.
% However, F1 scores of KAER on the dirty version of the dataset DBLP-GoogleScholar cannot compete with the results on the structured version (cleaner version). One reason might be that the misleading predictions based on the dirty input by CST result in semantic noise and propagate to the PLMs.
However, the F1 scores of all the other injections on the Dirty/DBLP-GoogleScholar cannot compete with the results on the baseline models (RoBERTa and Ditto). One reason might be that the misleading predictions based on the dirty input by CST result in semantic noise and propagate to the PLMs.
On the other hand, knowledge augmentation with PCT can advance the robustness of the model dealing with low-quality injections. For instance, \textbf{KAER (RoBERTa+CST+PCT)} obtains better F1 score than \textbf{KAER (RoBERTa+CST)} (72.00\% vs. 62.96\%). 
Similar improvement applies to \textbf{KAER (RoBERTa+EL+PCT)} vs. \textbf{KAER (RoBERTa+EL)} %(77.78\% vs 50.00\%), 
and  \textbf{KAER (RoBERTa+CST+EL+PCT)} vs. \textbf{KAER (RoBERTa+CST+EL)}. %(71.11\% vs. 47.06\%).

% \textbf{KAER (RoBERTa+EL+PCT)}, and  on Dirt/iTunes-Amazon  improve the F1 score comparing with corresponding knowledge injection methods with and \textbf{KAER (RoBERTa+CST)}, , and \textbf{KAER (RoBERTa+CST+EL)}.
%, which verifies the importance and necessity of knowledge augmentation for better language understanding on entity resolution tasks.


% The prediction performance of our model heavily relies on the quality of the input dataset, in particular, the semantic column types based on the characteristics of the input data.  
 

% For instance, the dirty version of the iTunes-Amazon dataset is generated from the clean version by randomly emptying attributes and appending their values to another randomly selected
% attribute \cite{li_deep_2020}.
% \textit{Cascading error from knowledge injector leads to lower performance.} 
% xxx


==> 10experiments-copy-accuracy.tex <==
% TODO: dataset statistic table
\subsection{Dataset}

KAER is evaluated on the Magellan datasets \cite{magellandata} across various domains. 
%The data collection contains datasets designed for entity matching tasks . 
The overview of the datasets used in this study is shown in Table~\ref{tab:dataset_overview}. 
The Magellan datasets contain three types of datasets: dirty dataset, structured dataset, and textual dataset.
The dirty dataset is generated from the structured dataset by randomly removing attribute values and appending the initial values to another randomly selected attribute~\cite{li_deep_2020}.

\begin{table}[h]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lclccc}
\hline
\textbf{Data Type} & \textbf{Dataset} & \textbf{Domain} & \textbf{Size} & \textbf{\# Positive} & \textbf{\# Attr.} \\ \hline
Structured             & Amazon-Google      & software & 11,460 & 1,167 & 3 \\
                       & iTunes-Amazon      & music    & 539    & 132   & 8 \\
                       & DBLP-ACM           & citation & 12,363 & 2,220 & 4 \\
                       & DBLP-GoogleScholar & citation & 28,707 & 5,347 & 4 \\ \hline
\multirow{3}{*}{Dirty} & iTunes-Amazon      & music    & 539    & 132   & 8 \\
                       & DBLP-ACM           & citation & 12,363 & 2,220 & 4 \\
                       & DBLP-GoogleScholar & citation & 28,707 & 5,347 & 4 \\ \hline
Textual                & Abt-Buy            & product  & 9,575  & 1,028 & 3 \\ \hline
\end{tabular}
}
\caption{Dataset Summary}
\label{tab:dataset_overview}
\vspace{-0.7cm}
\end{table}

% \subsection{Implementation Details}
% We use RoBERTa-base as the backbone model. 
\subsection{Results}
The experimental results are presented in Table \ref{tab:injection_results}.

\textit{Knowledge augmentation performs better on smaller datasets.}
According to the experimental results, incorporating external knowledge can improve the performance on entity resolution tasks. In particular, the proposed knowledge augmentation methods outperform the two baseline models in a data-scarce context.
% This improvement is found to be more significant on datasets with a smaller amount of training data. 
% The results show that our proposed knowledge augmentation methods can improve the model performance over the state-of-the-art Ditto model, especially in a data-scarce context. 
% the F1 score of most knowledge injection methods and prompting methods are higher than the F1 score of baseline model Ditto 
For example, \textbf{KAER (RoBERTa+EL+/)} outperforms both baseline models Roberta and Ditto by 16.51\% and 17.43\% $\uparrow$ on dataset Structured/iTunes-Amazon significantly and 2.75\% and 8.26\% $\uparrow$ on dataset Dirty/iTunes-Amazon. The two baseline models perform worse on smaller datasets because the language model might not be able to learn enough information to distinguish between different entities when fine tuning, given fewer training instances correctly. 
 % \textit{Prompting with "/" performs better than space and K-BERT style injection.}
% Through prompting, the model is provided with additional knowledge to augment the learning process. The experimental results revealed that using slash ``/'' to prompt the model with additional knowledge performs better than using space and \textbf{P}rompting with \textbf{C}onstrained \textbf{T}uning (PCT) in most scenarios. For example, \textbf{KAER (RoBERTa+EL+/)} performs better than the other two prompting methods 
% %space and APE \textbf{KAER (RoBERTa+CST+EL)} and \textbf{KAER(RoBERTa+CST+EL+APE)} 
% on dataset Structured/DBLP-GoogleScholar. 
Prompting with PCT achieves better performance in datasets with smaller text lengths. For example, \textbf{KAER (RoBERTa+CST+PCT)} reaches the best accuracy (94.81\%), but not statistically significant on dataset Structured/Amazon-Google, which contains the smallest length of serialized data entry. Moreover, \textbf{KAER (RoBERTa+EL+PCT)} on Dirty/iTunes-Amazon makes a significant difference compared to Ditto, at 95\% confidence level.

\textit{Knowledge augmentation does not perform well on datasets from certain domains.}
The datasets used in our experiments span several different domains. Using our proposed knowledge augmentation methods (CST and EL), records from certain domains, such as music and online product, benefit from more accurate retrieved knowledge.
For example, \textbf{KAER (RoBERTa+CST+/)} achieves the highest accuracy, i.e., 98.43\%, on the Textual/Abt-Buy from the online product domain at 99\% confidence level compared with two baseline models.
\textbf{KAER (RoBERTa+EL+/)} and \textbf{KAER (RoBERTa+EL+PCT)} achieves the best accuracy (88.99\%) on the musical dataset Dirty/iTunes-Amazon. %As analyzed above, it outperforms both baseline models significantly. 
One potential reason for this notable improvement is that the entities mentioned in the datasets from these domains are more general.
However, publication datasets from domains like citation require more domain-specific or even expert knowledge rather than general commonsense. Our knowledge injection methods are primarily designed for retrieving general knowledge.
Thus, for datasets, like Structured/DBLP-ACM, \textbf{KAER (RoBERTa+CST+/)} achieves better accuracy (99.64\%) than the baseline models, but not significantly. Most KAER models achieve competitive performance than baselines on Structured/DBLP-ACM. For future improvement, additional external expert knowledge from the citation domain should be incorporated for knowledge injection. 
% \vt{The knowledge injection does not help in the highly domain-specific dataset. The knowledge we inject is not the correct knowledge in terms of the domain.}

\textit{Knowledge augmentation is affected by data quality.}
%We notice that 
KAER, with certain knowledge augmentation methods, outperforms the baseline models on dirty datasets. For instance, \textbf{KAER (RoBERTa+CST+EL)} slightly exceeds RoBERTa, and Ditto on Dirty/DBLP-GoogleScholar.
% However, F1 scores of KAER on the dirty version of the dataset DBLP-GoogleScholar cannot compete with the results on the structured version (cleaner version). One reason might be that the misleading predictions based on the dirty input by CST result in semantic noise and propagate to the PLMs.
However, the accuracy of most injections on the Dirty/DBLP-GoogleScholar cannot compete with the results on the baseline models (RoBERTa and Ditto). One reason might be that the misleading predictions based on the dirty input by CST result in semantic noise and propagate to the PLMs.
On the other hand, knowledge augmentation with PCT can advance the robustness of the model dealing with low-quality injections. For instance, \textbf{KAER (RoBERTa+CST+PCT)} obtains a better accuracy than \textbf{KAER (RoBERTa+CST)} (87.16\% vs. 81.65\%) on Dirty/iTunes-Amazon. 
Similar improvement applies to \textbf{KAER (RoBERTa+EL+PCT)} vs. \textbf{KAER (RoBERTa+EL)} 
and  \textbf{KAER (RoBERTa+CST+EL+PCT)} vs. \textbf{KAER (RoBERTa+CST+EL)}.

% \textbf{KAER (RoBERTa+EL+PCT)}, and  on Dirt/iTunes-Amazon  improve the F1 score comparing with corresponding knowledge injection methods with and \textbf{KAER (RoBERTa+CST)}, , and \textbf{KAER (RoBERTa+CST+EL)}.
%, which verifies the importance and necessity of knowledge augmentation for better language understanding on entity resolution tasks.


% The prediction performance of our model heavily relies on the quality of the input dataset, in particular, the semantic column types based on the characteristics of the input data.  
 

% For instance, the dirty version of the iTunes-Amazon dataset is generated from the clean version by randomly emptying attributes and appending their values to another randomly selected
% attribute \cite{li_deep_2020}.
% \textit{Cascading error from knowledge injector leads to lower performance.} 
% xxx


==> main-old/00abstract.tex <==
\begin{abstract}

Pre-trained language models have been widely applied and proven effective in various Natural Language Processing (NLP) tasks. Prior studies have also examined the possibility of using Pretrained Language Models (PLMs) for multiple data cleaning tasks, e.g., entity resolution (or entity matching). However, in reality, there are various challenges for the entity resolution tasks on real-world datasets, including heterogeneous formats, excessive length of data, and complicity of the semantic meaning within data. 
% 1. data from heterogeneous sources are in different format resulting in a messy input, 2. long sentences or descriptions that make it difficult to do the entity matching by simply calculating the distances between records, and 3. the semantic of data is not expressive enough to be understood by models without leveraging domain knowledge or referring to external entities.
% textual data contains references to external entities that are not explicitly mentioned within the data itself. 
In this study, we demonstrate how knowledge augmentation can be incorporated into PLMs without having to finetune the model at a high computational and labeling cost. 

\end{abstract}


==> main-old/01introduction.tex <==
% [What is entity resolution task, prior works …]

% Entity resolution is a significant problem and has been studied across many fields, such as database, data cleaning, machine learning and deep learning. Even though they are given different names across the studies, such as entity matching, record linkage, deduplication, merge/purge, and etc, the main goal is the same, which is trying to match(merge) multiple records that refer to the same real-world entity. 

Recent studies using \emph{Transformer-based pre-trained language models} (PLMs) have shown their strong ability in performing various types of NLP tasks \cite{min_recent_2021}. However, not many studies have discussed the application of PLMs in the domain of data cleaning. 

As a data cleaning task well-discussed by existing research, entity resolution aims to identify the entries referring to the same real-world entities within or across databases~\cite{christen_data_2012}. Entity resolution, also known as entity matching, record linkage, or data deduplication, is a classical problem in data integration~\cite{zhao_auto-em_2019}. The typical process of entity resolution contains data preparation, data indexing or blocking, and data matching. 
Christian (2012) mentioned that schema standardization of records is an essential data preparation for entity resolution task~\cite{christen_data_2012}. 
Koutmarelas et al. (2020) analyzed the effectiveness of multiple syntactic-level data preparations, e.g., tokenization or stemmization, for threshold-based classifiers~\cite{koumarelas_data_2020}. 

With transformer-based \emph{pre-trained language models} (PLMs), recent studies draw increasing attention to entity resolution problems by leveraging PLMs~\cite{li_deep_2020, trabelsi_dame_2022}. However, current studies show that the performance might not be ideal for simply inputting the serialized entity pairs into PLMs for classification. For example, Li et al. (2020) proposed a new model, Ditto, which injects domain information, i.e., an \emph{entity type}, and standardizes the numerical formats to improve the performance before feeding the serialized entity pairs into PLMs. Inspired by Ditto, semantic-level data preparations, like entity type injection, can contribute to the entity resolution problems. Moreover, 
% [Recent work of using PLMs for data cleaning]
% Entity resolution can be seen as one of the challenging data cleaning tasks.
in real-life data cleaning practice, the source data often cover varied domains (e.g., publications, online products, geolocations) and in different formats (e.g., numerical, textual, non/structured). All of these increase the difficulty for practitioners to perform entity resolution tasks without prior knowledge about the domain-specific information about the data.


% data cleaning tasks such as entity resolution without the prior knowledge about the domain-specific information about the data itself. 
Prior work has also shown that performing data preparation to clean the data before applying ML-based models for entity resolution can improve task performance \cite{koumarelas_data_2020}. However, it still remains under-studied how domain-specific knowledge can be incorporated into the input data, and how it can benefit downstream data cleaning tasks such as entity resolution.

	


\section{Research Problems}
In this project, we target the following research questions:
\begin{itemize}
    \item (RQ$_1$) How to incorporate domain knowledge into input data when using PLMs for data cleaning?
    
    \item (RQ$_2$) To what extent does the incorporation of domain knowledge benefit downstream data cleaning tasks, such as entity resolution? 
\end{itemize}

% ....TODO: finalize RQ1, RQ2

Starting from state-of-the-art methods using pre-trained language models, such as Ditto \cite{li_deep_2020}, and code for entity resolution tasks, we will first conduct a number of experiments to measure the performance, both in terms of result accuracy, e.g., F1 values, and computational efficiency through benchmarking experiments.

We will then enhance this state-of-the-art method by using column semantic type inference \cite{hulsebos_sherlock_2019} and entity linking \cite{ayoola_refined_2022} (i.e., semantic information using online resources such as Wikidata/Wikipedia), in order to inject domain-specific information as additional signals to pre-trained language models. 

\textbf{Notation of Entity Resolution Task}
We now describe the formulation of the entity resolution task we will focus on in this paper. The input of the entity resolution task consists of a set $M \subseteq D_1 \times D_2$ of data entries $e \in M$, where $D_1$ and $D_2$ are two sets of data entry collections that contain duplicated entries. 
For each data entry, $e \in {(attr_i, val_i)}_{1 \leq i \leq N}$ where $N$ is the size of the set $M$, and $(e_1, e_2) \in M$. The task discussed in this paper focuses on: for each data entry pair $(e_1, e_2) \in M$, determine whether this pair is a pair of duplicated data entries.
% \yiren{TODO}


==> main-old/02related-work.tex <==
\subsection{Data Preparation: a Preceding Stage of Entity Resolution}

Data quality impacts the cost and performance of entity resolution systems significantly. Even for an error-free system with perfectly clean data, data from multiple sources are often not saved in a consistent way or carefully controlled for quality \cite{elmagarmid_duplicate_2007}. Usually, the data preparation stage includes parsing, data transformation, and standardization steps, and the goal is to improve the quality of the in-flow data and make the data comparable, and more usable \cite{elmagarmid_duplicate_2007}. 

Even though adjusting and selecting data preparators to prepare data before doing the entity resolution is not the focus of this paper, we will still apply some general data transformations to deal with specific data types. Data transformations are used to convert the data into the correct type or format that conforms to their domains \cite{elmagarmid_duplicate_2007}. Enhancing data quality by preprocessing data also contributes to the result of Sherlock \cite{hulsebos_sherlock_2019}, which can detect the semantic data types. Here we mainly use general transformations to help normalize the atomic types of data, such as \textit{string}, \textit{integer}, \textit{Boolean}. For instance, the \textit{float} type of data values for $Year$ is meaningless. So a simple conversion of the data from \textit{float} to \textit{integer} is required. Meanwhile, encoding issues also appear across the data values that need to be addressed at this stage. For numerical data, range checking could be used to ensure that data is in the appropriate range \cite{elmagarmid_duplicate_2007}. Preprocessing composite data values will be more complicated that requires a few steps, i.e., we usually first split the data values and then prepare data values separately, and finally merge the cleaned data values.

\subsection{Schema Matching: The Context of Entity Resolution}
% Assigned to Lan Li
Entity resolution is to identify and match records that refer to the same real-world entity. In many situations, raw records are stored from heterogeneous sources, while most existing techniques on entity resolution predefine the same schema for records from different sources \cite{elmagarmid_duplicate_2007}. Moreover, records from different sources might follow different structures at the attribute level, which adds more difficulties for entity resolution tasks \cite{enriquez_entity_2017, arabnia_when_2021}. Therefore, schema matching is required to discuss before we talk about entity resolution tasks. In particular, we consider the schema matching task as the context of processing entity resolution for schema matching guides which two records should be paired at the column level before processing the entity resolution at the row level. \cite{lin_efficient_2020} perform schema matching by creating a \textit{full schema} in which they compare and merge records from different sources into \textit{super record} before the entity resolution. In this way, they avoid information loss during the schema-matching process.

The main operation in manipulating schema information is \textit{Match}, which inputs two schemas and produces a mapping between two elements of the two schemas that relate semantically to each other \cite{rahm_survey_2001}. \cite{rahm_survey_2001} select the matching algorithms (a.k.a matchers) based on the application domain and schema types, and use data types to constrain the search space of correspondences. 

\subsection{Pretrained Model for Entity Resolution}
% Assigned to Lan Li

\cite{zhao_auto-em_2019} propose a transfer-learning approach to entity matching (EM), leveraging pre-trained entity matching models that are based on large-scale, production knowledge bases (KB). Auto-EM enables entity type detection and entity matching at the attribute level by learning a large amount of data from KBs. In this way, they achieve a high EM quality with little labeled training data. \cite{wu_zeroer_2020} introduce ZeroER that requires \textit{Zero} labeled examples for entity resolution task. They leverage a powerful generative model based on Gaussian Mixture Models for learning the match and mismatch distributions. 

Unlike Recurrent Neural Network (RNN) used in (\cite{zhao_auto-em_2019}, \cite{mudgal_deep_2018}), a few recent work applies transformer-based PLMs to entity resolution tasks. Paganelli et al. analyzes that simply fine-tuning BERT for matching/non-matching classification task mainly updates the last layers of the BERT components and BERT can recognize the input sequence represents a pair of records~\cite{paganelli_analyzing_2022}. Li et al. leverages siamese network structure to PLMs in order to improve the efficiency of PLMs during blocking phase~\cite{li_improving_2021}. 
Ditto by \cite{li_deep_2020} is now the state-of-the-art entity matching system based on pre-trained Transformer-based language models. In addition, Ditto provides deeper language understanding for entity resolution by injecting domain knowledge, summarizing the key information, and augmenting with more difficult examples for training data. The method of conditioning the language model, a.k.a, "prompting," is a hot topic in Nature Language Processing \cite{kojima_large_2022}. They \cite{kojima_large_2022} propose Zero-shot-CoT, a single zero-shot prompt that evokes a chain of thought from large language models, highlighting that the performance of the language model has been affected by different templates of the prompt. 
% Auto-EM introduce the framework to pretrain an RNN-based attribute type classifier on large knowledge base .
\vspace{-0.5em}
\subsection{Knowledge augmentation}
There are existing studies about methods that can be used to inject external domain knowledge into PLMs: 

% \subsection{Semantic data types recognition at column-level}

\textbf{Semantic data types detection at column-level.}
Sherlock \cite{hulsebos_sherlock_2019} is a novel system that uses a deep learning approach to detect semantic data types at the column level. Sherlock predicts the conceptual domain of a column when there is no schema or the existing schema cannot provide a fine-grained description of the data. Doduo~\cite{suhara_annotating_2022} is another recent method for annotating  columns with semantic types and for adding semantic relations between columns. Both Sherlock and Doduo methods can be used to inject domain-specific knowledge for columns with existing names or missing names.


\textbf{Entity Linking:}
Entity Linking \cite{li_deep_2020} refers to the task of linking entity mentions appearing in natural language text with their corresponding entities in an external knowledge base, e.g., Wikidata. 

% Existing work using traditional methods for entity linking .... \yiren{TODO}

Existing study has explored using PLMs to perform entity linking tasks, and achieved promising results. 
Zhang et al.'s work \cite{zhang_ernie_2019} introduced the model ERNIE by jointly pre-training BERT with a masked language modeling objective. The knowledge augmented BERT model is found to outperform existing methods in multiple knowledge-driven tasks. 
Later work by Peter et al. \cite{peters_knowledge_2019} futher improved the ERNIE model by introducing a trainable entity linker module and alignment between entity embedding and BERT embedding. 
Recent work by Ayoola et al. \cite{ayoola_refined_2022} introduced an entity linking method by using fine-tuning a pre-trained language model over Wikipedia data. The model has shown strong ability in zero-shot domain adaptation, which is used as a baseline method for entity linking in our study. 

\textbf{Knowledge Incorporation} %\liri{Liri}
Recent works shows that injecting external knowledge to PLMs can benefit Natural Language Reprocessing (NLP) downstream tasks~\cite{zhang_ernie_2019,peters_knowledge_2019,liu_k-bert_2020,wang_k-adapter_2021, wang_kepler_2021}. Furthermore, the method to inject the identified external knowledge into PLMs matters. Liu et al. propose the model K-BERT adding soft-position encoding and visible matrix to the augmented input sequence to avoid exposing too much knowledge to the original input and corresponding models~\cite{liu_k-bert_2020}. Another direction of knowledge incorporation is to align the knowledge embedding and PLMs output into same embedding space. The work from Wang et al. \cite{wang_kepler_2021} introduced a joint pre-training method based on roBERTa to map knowledge base entity and natural language entity description into the sample space. The knowledge embedding produced by KEPLER can be utilized as an additional input information source in our entity resolution task. K-Adaptor, proposed by Wang et al.~\cite{wang_k-adapter_2021}, stacks pre-trained multiple adapter model with RoBERTa for different types of knowledge, e.g. one for factual knowledge from knowledge base and another for linguistic-related syntax knowledge. The effectiveness of these methods in incorporating knowledge into entity resolution tasks can be further explored.

==> main-old/03potential-solutions.tex <==
We plan to examine several potential methods that can improve the task performance of entity resolution. 
First, we want to investigate whether the incorporation of additional external knowledge (e.g., WikiData) can help improve PLMs' ability in handling entity resolution tasks; Second, we want to propose a new method to better incorporate useful information as a signal for entity resolution.

We will experiment on thirteen open-access datasets used by DeepMatcher~\cite{mudgal_deep_2018} and Ditto~\cite{li_deep_2020}. We summarize the statistics of these datasets in Table~\ref{tab:exp-data}.


\begin{table}[h]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|l|c|c|c|c|}
\hline
\textbf{Data Type}          & \multicolumn{1}{c|}{\textbf{Datasets}} & \textbf{Domains} & \textbf{Size} & \textbf{\# Positive} & \textbf{\# Attributes} \\ \hline
\multirow{7}{*}{Structured} & Amazon-Google                          & software         & 11,460        & 1,167                & 3                      \\ \cline{2-6} 
                            & Walmart-Amazon                         & electronics      & 10,242        & 962                  & 5                      \\ \cline{2-6} 
                            & DBLP-Scholar                           & citation         & 28,707        & 5,347                & 4                      \\ \cline{2-6} 
                            & DBLP-ACM                               & citation         & 12,363        & 2,220                & 4                      \\ \cline{2-6} 
                            & iTunes-Amazon                          & music            & 539           & 132                  & 8                      \\ \cline{2-6} 
                            & BeerAdvo-RateBeer                      & beer             & 450           & 68                   & 4                      \\ \cline{2-6} 
                            & Fodors-Zagats                          & restaurant       & 946           & 110                  & 6                      \\ \hline
\multirow{2}{*}{Textual}    & Abt-Buy                                & product          & 9,575         & 1,028                & 3                      \\ \cline{2-6} 
                            & Company                                & company          & 112,632       & 28,200               & 1                      \\ \hline
\multirow{4}{*}{Dirty}      & iTunes-Amazon                          & music            & 539           & 132                  & 8                      \\ \cline{2-6} 
                            & DBLP-ACM                               & citation         & 12,363        & 2,220                & 4                      \\ \cline{2-6} 
                            & DBLP-Scholar                           & citation         & 28,707        & 5,347                & 4                      \\ \cline{2-6} 
                            & Walmart-Amazon                         & electronics      & 10,242        & 962                  & 5                      \\ \hline
\end{tabular}%
}
\caption{Datasets summary}
\label{tab:exp-data}
\end{table}
We have created and implemented the experimental framework, and performed several initial experiments as a proof of concept. The preliminary results are encouraging and seem to support our hypothesis, i.e.,  that introducing additional knowledge can improve the performance of using PLMs for entity resolution. Additionally, we also find that additional domain knowledge introduced has exhibited a stronger improvement over ER tasks with a relatively limited amount of available training data (as in Table 1, iTunes-Amazon).
	
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!h]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|ccc}
\hline
                       & \multicolumn{3}{c}{\textbf{Datasets}}                                                                                                                                                                                         \\ \hline
                       & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}DBLP-GoogleScholar \\ (N=17,223)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Abt-Buy \\ (N=5,743)\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}iTunes-Amazon\\ (N=321)\end{tabular}} \\ \hline
Ditto                  & \multicolumn{1}{c|}{0.944}                               & \multicolumn{1}{c|}{0.824}                                                               & 0.625                                                                    \\ \hline
Ditto + EL & \multicolumn{1}{c|}{0.946}                               & \multicolumn{1}{c|}{0.831}                                                               & 0.720                                                                    \\ \hline
\end{tabular}%
}
\caption{Preliminary experimental results (F1 scores): entity linking exhibits more improvements over smaller datasets.}
\label{tab:exp-results}
\end{table}
% Table 1. preliminary experiment results (F1 scores); Entity linking exhibits better improvement over smaller dataset;


